Improving Policy Optimization via $\varepsilon$-Retrain

We present $\varepsilon$-retrain, an exploration strategy encouraging a behavioral preference while optimizing policies with monotonic improvement guarantees. To this end, we introduce an iterative procedure for collecting retrain areas -- parts of the state space where an agent did not satisfy the behavioral preference. Our method switches between the typical uniform restart state distribution and the retrain areas using a decaying factor $\varepsilon$, allowing agents to retrain on situations where they violated the preference. We also employ formal verification of neural networks to provably quantify the degree to which agents adhere to these behavioral preferences. Experiments over hundreds of seeds across locomotion, power network, and navigation tasks show that our method yields agents that exhibit significant performance and sample efficiency improvements.

==> package.tex <==
\usepackage{balance} % for balancing columns on the final page

\usepackage{mathtools}          % Extends amsmath, providing common math tools
\usepackage{mathrsfs}   

%%%%%%%%%% emarche %%%%%%%%%%
% Enables \mathscr, which can work in cases that \mathcal does not
%\mathtoolsset{showonlyrefs}     % Only number equations that are referenced (optional)
\usepackage{graphicx}           % For including images
\usepackage{subcaption}         % Allows for the use of subfigures and subcaptions
\usepackage[space]{grffile}     % For spaces in image names
\usepackage{url}                % For displaying urls
\usepackage{booktabs} % for professional tables
\usepackage{wrapfig}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{multicol}
\usepackage{makecell}
\usepackage[bottom]{footmisc} 

\newcommand{\emarche}[1]{\color{blue}{[EM]: #1}}

\newcommand{\ourmethod}{\textit{$\varepsilon$-retrain}}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

==> sections/experiment_old.tex <==
\section{Experiments}
\label{sec:experiments}
This section presents a comprehensive evaluation of \ourmethod~applied to TRPO \citep{TRPO} that approximates the policy optimization theory of Section \ref{sec:method_theory}, and PPO \citep{PPO} which relaxes the computational demands of TRPO, resulting in a simple yet well-performing algorithm. We refer to these methods as $\varepsilon$-TRPO and $\varepsilon$-PPO. Additionally, we investigate the impact of the proposed approach on the CMDP framework \citep{altman1999cmdp}, using the Lagrangian method on top of TRPO and PPO to model behavioral preferences as constraints. The resulting algorithms are named TRPOLagr, PPOLagr, $\varepsilon$-TRPOLagr, and $\varepsilon$-PPOLagr.

Our experiments address the following key questions: (i) \textit{Does \ourmethod~allow agents to better adhere to behavioral preferences while solving the task?} (ii) \textit{How does \ourmethod~impact existing CMDP-based methods aimed at satisfying these preferences?} (iii) \textit{How often do agents satisfy the behaviors provably and empirically?} To answer these questions, we begin our experiments using two known safety-oriented tasks, SafetyHopperVelocity-v1, and SafetyHalfCheetahVelocity-v1, from the Safety-Gymnasium benchmark \citep{SafetyGymnasium}. To evaluate our method in a variety of setups and different behavioral desiderata, we also employ two practical scenarios based on an active network management task for a power system \citep{gymanm}, and navigation for a mobile robot \citep{drl_navigation1,drl_navigation2}. These tasks are {\color{red}described in detail in Sec.\ref{subsec:envs} in the supplementary material and} depicted in Figure \ref{fig:envs}. For simplicity, we will refer to them as \textit{Hopper}, \textit{HalfCheetah}, \textit{Active Network Management} and \textit{Navigation}, respectively.

\begin{figure}[h!]
    \centering
    \begin{minipage}[b]{0.17\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/hopper.png}
        \label{fig:hopper}
        \text{(a) Hopper}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.17\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/halfcheetah.png}
        \label{fig:cheetah}
        \text{(b) HalfCheetah}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/anm.png}
        \label{fig:anm}
        \text{(c) Active Network Management}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.17\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/navigation.png}
        \label{fig:nav}
        \text{(d) Navigation}
    \end{minipage}
    \caption{Environments employed in the empirical evaluation of \ourmethod.}
    \label{fig:envs}
\end{figure}


\subsection{Implementation Details.}
\label{sec:implementation_details}
Data collection is performed on Xeon E5-2650 CPU nodes with 64GB of RAM, using existing implementations for PPO, TRPO, and their Lagrangian, based on the omnisafe library \citep{ji2023omnisafe}. Complete hyperparameters are in Appendix \ref{app:hyperparameters}. To ensure statistical significance \citep{colas2019eval}, we report the average return, cost, and standard error as shaded regions over the last training epoch of 50 independent runs per method. Figures \ref{fig:base_results} and~\ref{fig:lag_results} show the average return in the first row, and the average cost in the second row, where each column represents a different task. Notably, \textit{we are seeking agents that achieve a lower cost, which indicates they better adhere to the desired behavioral preferences}. Our claims on the performance improvement of \ourmethod~are supported by 1600 training runs.%\footnote{While some of the results indicate the algorithms have not converged yet, we enforced a strict 24-hour limit on the training of the agents due to the high number of runs.}
This number of independent trials significantly surpasses the typical 3-10 runs per method used in previous policy optimization works \citep{TRPO,PPO}, motivating different results compared to the published baselines {\lmarza{Here maybe we should say that we use a penalty in the reward function. Hence, the results are not directly comparable with the original baseline...}}. Considering the computational resources used for our experiments, Appendix \ref{app:env_impact} also addresses the environmental impact. % and our strategy to offset estimated CO$_2$ emissions.

\subsection{Empirical Evaluation}
%\emarche{TODO: Experiments with varying parameters for \ourmethod} \\
\textbf{Performance of $\varepsilon$-TRPO and $\varepsilon$-PPO.} Figure \ref{fig:base_results} shows that TRPO and PPO enhanced with our \ourmethod~improve sample efficiency and allow agents to better adhere to the behavioral preferences.
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/results_base.png}
    \vspace{-5pt}
    \caption{Comparison of $\varepsilon$-PPO, $\varepsilon$-TRPO, PPO and TRPO in four different environments. Each column (i.e., each task) shows the average reward and cost during the training.}
    \label{fig:base_results}
\end{figure}
In Hopper and HalfCheetah, both TRPO and PPO achieve substantially higher returns compared to their \ourmethod\;version; a result that could be easily misunderstood. In fact, this is related to the nature of the task, where the reward is directly proportional to the agents' velocities.\footnote{Notably, the lower velocity limit of the Hopper task causes a linear relationship between average return and cost: the two functions grow in the same way.} For this reason, an agent that violates the behavioral preference \textit{``limit velocity under a threshold''}, achieves higher returns. This is clearly shown in the bottom row depicting the average cost, where $\varepsilon$-TRPO and $\varepsilon$-PPO resulted in notably lower cost compared to the baselines, indicating they lead the agents towards adhering to the velocity limit significantly more often than TRPO and PPO. Conversely, in the active network management task $\varepsilon$-TRPO is notably more sample efficient over TRPO, achieving the same performance in $\approx50\%$ of the training steps. $\varepsilon$-PPO also achieves both lower cost and higher return than PPO. At a high level, violating the operational constraints leads to higher penalties and inferior returns, and \ourmethod-enhanced algorithms learn how to operate the grid successfully (i.e., not violating operational constraints but suffering natural energy losses) using a fraction of the training steps of the baselines. The benefits of \ourmethod~are also confirmed in the navigation task, where violating the safety desiderata \textit{``avoid collisions''} leads to more collisions. Ultimately, achieving a higher cost (i.e., more collisions) hinders the navigation performance of the agent and leads to inferior returns. Specifically, TRPO and $\varepsilon$-TRPO converge to the same average cost. However, the higher sample efficiency of the latter through the training, in terms of learning collision avoidance behaviors more quickly, allows $\varepsilon$-TRPO to learn better navigation behaviors, outperforming TRPO in terms of average return. Moreover, $\varepsilon$-PPO significantly outperforms PPO both in terms of average cost and return.

\textbf{Performance of $\varepsilon$-TRPOLagr and $\varepsilon$-PPOLagr.} 
Lagrangian-based methods have been recently employed for encouraging behavioral preferences in policy optimization \citep{julien2022behavioralspec}. Here, we analyze the impact of \ourmethod~on these CMDP-based methods, modeling our desiderata as constraints.
\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{images/results_lag_new.png}
    \vspace{-5pt}
    \caption{Comparison of $\varepsilon$-PPOLagr, $\varepsilon$-TRPOLagr, PPOLagr and TRPOLagr in four different environments. Each column (i.e., each task) shows the average reward and cost during the training.}
    \label{fig:lag_results}
\end{figure}
Figure \ref{fig:lag_results} shows that constrained policy optimization algorithms enhanced with \ourmethod~reduce the constraint violations and, in the more complex tasks, allow agents to improve performance.
During training, both $\varepsilon$-TRPOLagr and $\varepsilon$-PPOLagr drastically reduce the amount of constraint violations in the Hopper and HalfCheetah velocity environments. We specify the fraction of training steps where agents violate their constraint in Table \ref{tab:violation_perc}.
However, at convergence, all the approaches satisfy the imposed thresholds. These results lead to a couple of interesting considerations based on the setup of interest. In safety-critical contexts where it is crucial to satisfy constraints at training time, \ourmethod~showed significant empirical benefits. On the other hand, in non-critical contexts where performance at convergence is the main evaluation metric, the naive Lagrangian methods have superior return performance. Intuitively, this relates to the fact that Lagrangian methods often violate the constraints at training time, allowing agents to explore more and thus learn higher-performing behaviors.
In the more complex, realistic scenarios, our empirical analysis leads to different considerations. 
\begin{table}[t]
\centering
\vspace{-5pt}
\caption{Average fraction of the training steps where agents violate the constraints (lower is better).}
\begin{tabular}{ccccc}
\toprule
    & \textbf{Hopper} & \textbf{HalfCheetah} & \textbf{Active Network Management} & \textbf{Navigation} \\ \midrule
\textbf{PPOLagr}                & 0.57   & 0.33        & \textbf{0.44}                      & 0.46       \\
\textbf{$\varepsilon$-PPOLagr}  & \textbf{0.04}   & \textbf{0}           & 0.59                      & \textbf{0.44}       \\\midrule
\textbf{TRPOLagr}               & 0.51   & 0.17        & \textbf{0.58}                      & 0.64       \\ 
\textbf{$\varepsilon$-TRPOLagr} & \textbf{0.25}   & \textbf{0}           & 0.79                      & \textbf{0.56}       \\
\bottomrule
\end{tabular}
\label{tab:violation_perc}
\end{table}
Specifically, in navigation, \ourmethod-based methods and the Lagrangian baselines achieve comparable results in terms of cost (i.e., constraint satisfaction). However, retraining agents on areas that are collision-prone, allowed the agents to learn policies with better navigation skills and higher performance. The benefits of retraining agents in areas of interest are further confirmed in the active network management task. In particular, the Lagrangian baselines fail to solve the problem successfully. In contrast, our empirical results suggest that retraining agents in situations where the power grid becomes unstable can ultimately lead agents to learn how to successfully operate the grid.


\textbf{Verifying Navigation Behaviors Provably.} 

\begin{figure}[b]
    \begin{minipage}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/density_nav_init.png}
        \par\vspace{15pt}
    \end{minipage}%
    \hspace{1pt}
    \begin{minipage}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\textwidth]{images/density_nav_end.png}
        \par\vspace{15pt}
    \end{minipage}%
    \hspace{10pt}
    \begin{minipage}[b]{0.3\textwidth}
        \input{sections/table}
        \par\vspace{-2pt}
    \end{minipage}
\caption{(left) Density map of the retrain areas collected in the first and last epochs of training; yellow indicates higher density. (right) Average behavioral violations percentage for policies trained with TRPO, PPO, PPOLagr, TRPOLagr, and their \ourmethod\;version.}
\label{tab:resultsFV}
\end{figure}

To further assess the benefit that \ourmethod~has over the behavioral preferences, we formally verify the policies trained for the navigation task. We consider this problem as an explanatory task for clarity since it allows us to easily visualize the retrain areas generated for \textit{``collision avoidance''} on top of the environment. Figure \ref{tab:resultsFV} on the left, shows a kernel density estimation map of the retrain areas distribution at the beginning (left) and final stages (right) of the training for the $\varepsilon$-TRPO agent. Here we can notice how the agent successfully learns to navigate the environment over time since the retrain areas are more equally distributed through the entire scenario.

Using the verification tool proposed by \citet{CountingProVe}, we aim to quantify the probability that a navigation policy violates the collision avoidance preference. 
To this end, we consider three representative retrain areas collected while training the different \ourmethod-based algorithms (depicted as red dots in Figure \ref{tab:resultsFV}). For each area, we encode the input-output relationship required by the tool (see Section \ref{sec:verification}), considering the retrain area as the precondition, and the minimum linear and angular velocities that would cause a collision as the postcondition. Broadly speaking, the FV tool checks where the trained policies do not exceed such minimum velocities (i.e., they do not collide), and returns the portion of each retrain area for which the given policy violates the postcondition (i.e., the probability of colliding in that area). 
Table \ref{tab:resultsFV} reports the probability that policies at convergence collide in the chosen retrain areas, averaged over all the runs. Overall, this additional analysis based on FV highlights that \ourmethod-enhanced algorithms better adhere to the behavioral preference, further confirming our intuitions and the merits of our approach.  

% show that although policies at convergence empirically achieve a comparable amount of collisions (see Figure \ref{fig:base_results}, \ref{fig:lag_results}, 

%thus making it difficult to state which one better respects specific desiderata, exploiting formal verification, it is possible to formally
%For each retrain area selected, we define a specific safety property (i.e., a behavioral preference in terms of \textit{collision avoidance}) setting for the precondition, the agent's input features encoded using the intervals collected online during training, while for the postcondition (i.e., the action to be avoided) the minimum linear and angular velocity allowed before a collision in that specific region\footnote{We note that thanks to the simulated environment it is possible to visualize each retrain area after its collection and thus given a specific agent's position centered in the area, compute the minimum linear and angular velocity allowed before a collision by exploiting the simulator physics engine.}. 




==> sections/table.tex <==
\tiny
\begin{tabular}{@{\extracolsep{-5pt}}ccccc}
 \toprule &\multicolumn{3}{c}{\textbf{Retrain areas (1, 2, 3)}} 
\\
\midrule 
 \makecell[l]{$\varepsilon $-PPO\\PPO} & \makecell[l]{\textbf{0.007\%}\\0.012\%}  & \makecell[l]{\textbf{0.011\%}\\0.017\%} & \makecell[l]{\textbf{0.22\%}\\0.59\%} \\
\midrule 
 \makecell[l]{$\varepsilon $-TRPO\\TRPO} & \makecell[l]{\textbf{0.014\%}\\0.015\%} & \makecell[l]{\textbf{0.67\%}\\0.69\%} & \makecell[l]{1\%\\\textbf{0.8\%}}  \\
\midrule 
 \makecell[l]{$\varepsilon $-PPOLagr\\PPOLagr} &\makecell[l]{\textbf{0.006\%}\\0.013\%} & \makecell[l]{\textbf{0\%}\\0.05\%} & \makecell[l]{\textbf{0.012\%}\\0.1\%}  \\
\midrule 
 \makecell[l]{$\varepsilon $-TRPOLagr\\TRPOLagr} & \makecell[l]{0.0004\%\\\textbf{0.00005\%}} & \makecell[l]{\textbf{0.007\%}\\0.012\%} & \makecell[l]{\textbf{0.46\%}\\0.48\%}  \\
\midrule 
\end{tabular}

%\caption{Mean \textit{violation rate} during 25 epochs of training considering TRPO, PPO, PPOLagr, TRPOLagr, and the respective \ourmethod\;version using different random seeds.}
 \label{tab:resultsFV}


==> sections_old/discussion.tex <==
\section{Discussion}

This work presented \ourmethod, a novel exploration strategy with monotonic improvement guarantees that optimizes policies while encouraging specific behavioral preferences. Our approach aims at retraining an RL agent from \textit{retrain areas} where it violated a desired behavioral preference at training time. 
%In detail, we used an $\varepsilon$ decay strategy to combine the uniform restart state distribution over the state space, typical of RL algorithms, with a restart strategy over retrain areas that are collected and refined during training. Crucially, we also derived a novel bound on the monotonic policy improvement of policies optimized via these mixed restart distributions that motivate our design choices and the superior performance of \ourmethod~enhanced algorithms.
Our empirical and formal evaluation over hundreds of seeds considering various tasks and behavioral preferences, demonstrated the effectiveness in terms of higher sample efficiency and superior performance of \ourmethod~when integrated with existing policy optimization methods. Real-world experiments confirmed the benefit of the proposed approach in realistic setups. 

%, as well as Lagrangian approaches designed to enforce desired behaviors. In particular, we observe significantly higher sample efficiency, superior performance, and improved adherence to behavioral preferences, highlighting the impact of our approach in practical applications. Moreover, we utilized a verification tool to provably assess the degree to which trained policies adhere to the desiderata and transfer the learned policy to a real robot to further investigate the benefit of the proposed approach in realistic setups. 

%Notably, \ourmethod\;presents a mixed restart strategy that can be integrated with RL algorithms and opens up interesting avenues for its integration within emerging exploration techniques. Moreover, we believe our method provides a building block for developing novel solutions aimed at enforcing desired characteristics into RL-trained policies.

==> sections_old/experiment.tex <==
\section{Experiments}
\label{sec:experiments}

We present a comprehensive evaluation of \ourmethod~applied to TRPO \citep{TRPO} that approximates the policy optimization theory of Section \ref{sec:method_theory}, and PPO \citep{PPO} which relaxes the computational demands of TRPO. We refer to these methods as $\varepsilon$-TRPO and $\varepsilon$-PPO. Additionally, we investigate the impact of the proposed approach on the CMDP framework \citep{altman1999cmdp}, using the Lagrangian method on top of TRPO and PPO to model behavioral preferences as constraints. The resulting algorithms are named TRPOLagr, PPOLagr, $\varepsilon$-TRPOLagr, and $\varepsilon$-PPOLagr.\\
Our experiments address the following questions: (i) \textit{does \ourmethod~allow agents to better adhere to behavioral preferences while solving the task?} (ii) \textit{How does \ourmethod~impact existing CMDP-based methods aimed at satisfying these preferences?} (iii) \textit{How often do agents satisfy the behaviors provably and empirically?} To answer these questions, we begin our experiments using two known safety-oriented tasks, \textit{SafetyHopperVelocity-v1}, and \textit{SafetyHalfCheetahVelocity-v1}, from the Safety-Gymnasium benchmark \citep{SafetyGymnasium}. To evaluate our method in a variety of setups and different behavioral desiderata, we also employ two practical scenarios based on an active network management task for a power system \citep{gymanm}, and navigation for a mobile robot \citep{drl_navigation1,drl_navigation2}. These tasks are described in detail in Sec.\ref{subsec:envs} in the supplementary material. For simplicity, we will refer to them as \textit{Hopper} (Hop), \textit{HalfCheetah} (Che), \textit{Active Network Management} (ANM) and \textit{Navigation} (Nav), respectively.

\textbf{Implementation Details.}
\label{sec:implementation_details}
Data collection is performed on Xeon E5-2650 CPU nodes with 64GB of RAM, using existing implementations for PPO, TRPO, and their Lagrangian, based on the omnisafe library \citep{ji2023omnisafe}. Complete hyperparameters are in Appendix \ref{app:hyperparameters}. To ensure statistical significance \citep{colas2019eval}, we report the average return, cost, and standard error as shaded regions over the last training epoch of 50 independent runs per method. Figures~\ref{fig:base_results} and \ref{fig:lag_results} (the latter reported in the supplementary) show the average return in the first row and the average cost in the second row, where each column represents a different task. Notably, \textit{we are seeking agents that achieve a lower cost, which indicates they better adhere to the desired behavioral preferences}. Our claims on the performance improvement of \ourmethod~are supported by 1600 training runs, which significantly surpasses the typical 3-10 runs per method used in previous policy optimization works \citep{TRPO,PPO}. We remark that due to employing a small penalty in the reward function to encourage specific behavioral preference, our results are not directly comparable to the published baselines \citep{TRPO, PPO}. For a fair comparison, we first collect the baseline with this new setting and then compare the performance with our approach. Considering the computational resources used for our experiments, Appendix \ref{app:env_impact} also addresses the environmental impact. % and our strategy to offset estimated CO$_2$ emissions.

\textbf{Empirical Evaluation (Performance of $\varepsilon$-TRPO and $\varepsilon$-PPO).} Figure \ref{fig:base_results} shows that TRPO and PPO enhanced with our \ourmethod~improve sample efficiency and allow agents to better adhere to the behavioral preferences.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/results_base.png}
    \vspace{-5pt}
     \caption{Comparison of $\varepsilon$-PPO, $\varepsilon$-TRPO, PPO and TRPO in four different environments.} %Each column (i.e., each task) shows the average reward and cost during the training.}
    \label{fig:base_results}
    \vspace{-5mm}
\end{figure}
In Hopper and HalfCheetah, TRPO and PPO achieve substantially higher returns than their \ourmethod\;version; a result that could be easily misunderstood. In fact, this is related to the nature of the task, where the reward is directly proportional to the agents' velocities. %\footnote{Notably, the lower velocity limit of the Hopper task causes a linear relationship between average return and cost: the two functions grow in the same way.} 
For this reason, an agent that violates the behavioral preference \textit{``limit velocity under a threshold''}, achieves higher returns. This is clearly shown in the first two columns of Figure \ref{fig:base_results}, where $\varepsilon$-TRPO and $\varepsilon$-PPO resulted in notably lower cost compared to the baselines, indicating they lead the agents towards adhering to the velocity limit significantly more often than TRPO and PPO. Similar results are achieved in the ANM task where $\varepsilon$-TRPO and $\varepsilon$-PPO are notably safer and more sample efficient (see Pareto frontiers for convergence results in Figure \ref{fig:base_results_pareto} in the supplementary) than the baseline counterparts. 
%Conversely, in the active network management task, $\varepsilon$-TRPO is notably more sample efficient over TRPO, achieving the same performance in $\approx50\%$ of the training steps. $\varepsilon$-PPO also achieves both lower cost and higher return than PPO. 
%At a high level, violating the operational constraints leads to higher penalties and inferior returns, and \ourmethod-enhanced algorithms learn how to operate the grid successfully (i.e., not violating operational constraints but suffering natural energy losses) using a fraction of the training steps of the baselines. 
The benefits of \ourmethod~are also confirmed in the navigation task, where violating the safety desiderata \textit{``avoid collisions''} leads to more collisions. Ultimately, achieving a higher cost (i.e., more collisions) hinders the navigation performance of the agent and leads to inferior returns. Specifically, TRPO and $\varepsilon$-TRPO converge to the same average cost. However, the higher sample efficiency of the latter through the training, in terms of learning collision avoidance behaviors more quickly, allows $\varepsilon$-TRPO to learn better navigation behaviors, outperforming TRPO in terms of average return. Moreover, $\varepsilon$-PPO significantly outperforms PPO both in terms of average cost and return. 

\textbf{Performance of $\varepsilon$-TRPOLagr and $\varepsilon$-PPOLagr.} 
%Lagrangian-based methods have been recently employed for encouraging behavioral preferences in policy optimization \citep{julien2022behavioralspec}. Here, we analyze the impact of \ourmethod~on these CMDP-based methods, modeling our desiderata as constraints.
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{images/results_lag_new.png}
%     \vspace{-5pt}
%     \caption{Comparison of $\varepsilon$-PPOLagr, $\varepsilon$-TRPOLagr, PPOLagr and TRPOLagr in four different environments. Each column (i.e., each task) shows the average reward and cost during the training.}
%     \label{fig:lag_results}
% \end{figure}
% Figure \ref{fig:lag_results} shows that constrained policy optimization algorithms enhanced with \ourmethod~reduce the constraint violations and, in the more complex tasks, allow agents to improve performance.
During training (learning curves are reported
\begin{wraptable}{l}{0.55\textwidth}
%\begin{table}[t]
\vspace{-1mm}
\centering
\footnotesize
\begin{tabular}{ccccc}
\toprule
    & \textbf{Hop} & \textbf{Che} & \textbf{ANM} & \textbf{Nav} \\ \midrule
\textbf{PPOLagr}                & 0.57   & 0.33        & \textbf{0.44}                      & 0.46       \\
\textbf{$\varepsilon$-PPOLagr}  & \textbf{0.04}   & \textbf{0}           & 0.59                      & \textbf{0.44}       \\\midrule
\textbf{TRPOLagr}               & 0.51   & 0.17        & \textbf{0.58}                      & 0.64       \\ 
\textbf{$\varepsilon$-TRPOLagr} & \textbf{0.25}   & \textbf{0}           & 0.79                      & \textbf{0.56}       \\
\bottomrule
\end{tabular}
\caption{Average fraction of the training steps where agents violate the constraints (lower is better).}
\label{tab:violation_perc}
\vspace{-3mm}
%\end{table}
\end{wraptable}
 in Figure \ref{fig:lag_results} in the supplementary), both $\varepsilon$-TRPOLagr and $\varepsilon$-PPOLagr drastically reduce the amount of 
constraint violations in the Hopper and HalfCheetah velocity environments. We specify the fraction of training steps where agents violate their constraint in Table \ref{tab:violation_perc}. However, at convergence, all the approaches satisfy the imposed thresholds. These results lead to some interesting considerations based on the setup of interest. 
In safety-critical contexts where it is crucial to satisfy constraints at training time, \ourmethod~showed significant empirical benefits. On the other hand, in non-critical contexts where performance at convergence is the main evaluation metric, the naive Lagrangian methods have superior return performance. Intuitively, this relates to the fact that Lagrangian methods often violate the constraints at training time, allowing agents to explore more and thus learn higher-performing behaviors.
In the more complex, realistic scenarios, our empirical analysis leads to different considerations. 
Specifically, in navigation, \ourmethod-based methods and the Lagrangian baselines achieve comparable results in terms of cost (i.e., constraint satisfaction). However, retraining agents in areas that are collision-prone allowed them to learn policies with better navigation skills and higher performance. %The benefits of retraining agents in areas of interest are further confirmed in the ANM task. 
In the ANM task, retraining an agent during grid instability increases the frequency of constraint violations compared to the baseline. Nonetheless, our approach helps agents learn to manage the grid effectively over time in contrast to Lagrangian baselines, which in the end, fails to solve the problem efficiently (see the Pareto frontier in the supplementary material).
% In particular, the Lagrangian baselines fail to solve the problem successfully. In contrast, our empirical results suggest that retraining agents when the power grid becomes unstable can ultimately lead agents to learn how to successfully operate the grid.


\textbf{Provably Verifying Navigation Behaviors.} 
% \begin{figure}[t]
%     \begin{minipage}[b]{0.2\textwidth}
%         \centering
%         \includegraphics[width=0.8\textwidth]{images/density_nav_init.png}
%         \par\vspace{10pt}
%     \end{minipage}%
%     \hspace{1pt}
%     \begin{minipage}[b]{0.2\linewidth}
%         \centering
%         \includegraphics[width=0.8\textwidth]{images/density_nav_end.png}
%         \par\vspace{10pt}
%     \end{minipage}%
%     \hspace{1pt}
%     \begin{minipage}[b]{0.2\textwidth}
%         \par\vspace{-15pt}
%         \input{sections/table}
%         \par\vspace{-2pt}
%     \end{minipage}
% \caption{(left) Density map of the retrain areas collected in the first and last training epochs; yellow indicates higher density. (right) Average behavioral violations percentage for policies trained with TRPO, PPO, PPOLagr, TRPOLagr, and their \ourmethod\;version.}
% \label{tab:resultsFV}
% \vspace{-3mm}
% \end{figure}
To further assess the benefit that \ourmethod~has over the behavioral preferences, we formally verify the policies trained for the navigation task. We consider this problem as an explanatory task for clarity since it allows us to easily visualize the retrain areas generated for \textit{``collision avoidance''} on top of the environment.
\begin{wrapfigure}{l}{0.6\textwidth}
  \begin{center}
  \vspace{-10pt}
\includegraphics[width=\linewidth]{images/FV+areas.pdf}
      \end{center}
    \vspace{-9pt}
    \caption{(left) Density map of the retrain areas collected in the first and last training epochs; yellow indicates higher density. (right) Average behavioral violations percentage for policies trained with TRPO, PPO, PPOLagr, TRPOLagr, and their \ourmethod\;version.}
    \label{tab:resultsFV}
    \vspace{-9pt}
\end{wrapfigure}
Figure \ref{tab:resultsFV} on the left, shows a kernel density estimation map of the retrain areas distribution at the beginning (left) and final stages (right) of the training for the $\varepsilon$-TRPO agent. Here we can notice how the agent successfully learns to navigate the environment over time since the retrain areas are more equally distributed through the entire scenario.
Using a recent verification tool \citep{CountingProVe}, we aim to quantify the probability that a navigation policy violates the collision avoidance preference. 
To this end, we consider three representative retrain areas collected while training the different \ourmethod-based algorithms (depicted as red dots in Figure \ref{tab:resultsFV}). For each area, we encode the input-output relationship required by the tool (see Section \ref{sec:verification}), considering the retrain area as the precondition, and the minimum linear and angular velocities that would cause a collision as the postcondition. Broadly speaking, the FV tool checks where the trained policies do not exceed such minimum velocities (i.e., they do not collide), and returns the portion of each retrain area for which the given policy violates the postcondition (i.e., the probability of colliding in that area). 
The table in Figure \ref{tab:resultsFV} reports the probability that policies at convergence collide in the chosen retrain areas, averaged over all the runs. Overall, this additional analysis based on FV highlights that \ourmethod-enhanced algorithms better adhere to the behavioral preference, further confirming our intuitions and the merits of our approach.  


\textbf{Real experiments.} 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.7\linewidth]{images/real_exp.pdf}
%     \caption{Real-world experiments.}
%     \label{fig:real_exp}
%     \vspace{-3mm}
% \end{figure}
To conclude our comprehensive evaluation, we perform an additional evaluation in realistic unsafe mapless navigation settings. Due to the similar performance at
\begin{wrapfigure}{r}{0.45\textwidth}
  \begin{center}
  \vspace{-12pt}
\includegraphics[width=0.9\linewidth]{images/real_exp.pdf}
      \end{center}
    \vspace{-6pt}
    \caption{Real-world experiments comparing
    $\varepsilon$-TRPO and TRPO in corner-case scenarios.}
    \label{fig:real_exp}
    \vspace{-10pt}
\end{wrapfigure}
 convergence for TRPO and $\varepsilon$-TRPO, we report the evaluation for these two approaches. Specifically, we compare $\varepsilon$-TRPO and TRPO in scenarios where the agent has either all or only partially occluded LiDAR information.
We hypothesize that if the agent is not exposed to multiple unsafe situations during the training, i.e., without an \ourmethod\;strategy, it is less likely to select a longer but safer trajectory, and eventually, the agent will prefer a straight trajectory leading to a collision. 
To this end, the Unity framework \cite{unity} we used to create the navigation task allows us to transfer the policies trained in simulation on ROS-enabled platforms such as our Turtlebot3 (Fig. \ref{fig:real_exp}). Hence, we test several corner-case situations, comparing the safer (from the formal verification results) trained agent at convergence for both $\varepsilon$-TRPO and TRPO. Realistic experimental results confirm our hypothesis, showing the benefit of retraining the agent in specific regions of the state space deemed unsafe (we refer to the video in the supplementary material).




==> sections_old/experiment_old.tex <==
\section{Experiments}
\label{sec:experiments}
This section presents a comprehensive evaluation of \ourmethod~applied to TRPO \citep{TRPO} that approximates the policy optimization theory of Section \ref{sec:method_theory}, and PPO \citep{PPO} which relaxes the computational demands of TRPO, resulting in a simple yet well-performing algorithm. We refer to these methods as $\varepsilon$-TRPO and $\varepsilon$-PPO. Additionally, we investigate the impact of the proposed approach on the CMDP framework \citep{altman1999cmdp}, using the Lagrangian method on top of TRPO and PPO to model behavioral preferences as constraints. The resulting algorithms are named TRPOLagr, PPOLagr, $\varepsilon$-TRPOLagr, and $\varepsilon$-PPOLagr.

Our experiments address the following key questions: (i) \textit{Does \ourmethod~allow agents to better adhere to behavioral preferences while solving the task?} (ii) \textit{How does \ourmethod~impact existing CMDP-based methods aimed at satisfying these preferences?} (iii) \textit{How often do agents satisfy the behaviors provably and empirically?} To answer these questions, we begin our experiments using two known safety-oriented tasks, SafetyHopperVelocity-v1, and SafetyHalfCheetahVelocity-v1, from the Safety-Gymnasium benchmark \citep{SafetyGymnasium}. To evaluate our method in a variety of setups and different behavioral desiderata, we also employ two practical scenarios based on an active network management task for a power system \citep{gymanm}, and navigation for a mobile robot \citep{drl_navigation1,drl_navigation2}. These tasks are {\color{red}described in detail in Sec.\ref{subsec:envs} in the supplementary material and} depicted in Figure \ref{fig:envs}. For simplicity, we will refer to them as \textit{Hopper}, \textit{HalfCheetah}, \textit{Active Network Management} and \textit{Navigation}, respectively.

\begin{figure}[h!]
    \centering
    \begin{minipage}[b]{0.17\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/hopper.png}
        \label{fig:hopper}
        \text{(a) Hopper}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.17\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/halfcheetah.png}
        \label{fig:cheetah}
        \text{(b) HalfCheetah}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/anm.png}
        \label{fig:anm}
        \text{(c) Active Network Management}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.17\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/navigation.png}
        \label{fig:nav}
        \text{(d) Navigation}
    \end{minipage}
    \caption{Environments employed in the empirical evaluation of \ourmethod.}
    \label{fig:envs}
\end{figure}


\subsection{Implementation Details.}
\label{sec:implementation_details}
Data collection is performed on Xeon E5-2650 CPU nodes with 64GB of RAM, using existing implementations for PPO, TRPO, and their Lagrangian, based on the omnisafe library \citep{ji2023omnisafe}. Complete hyperparameters are in Appendix \ref{app:hyperparameters}. To ensure statistical significance \citep{colas2019eval}, we report the average return, cost, and standard error as shaded regions over the last training epoch of 50 independent runs per method. Figures \ref{fig:base_results} and~\ref{fig:lag_results} show the average return in the first row, and the average cost in the second row, where each column represents a different task. Notably, \textit{we are seeking agents that achieve a lower cost, which indicates they better adhere to the desired behavioral preferences}. Our claims on the performance improvement of \ourmethod~are supported by 1600 training runs.%\footnote{While some of the results indicate the algorithms have not converged yet, we enforced a strict 24-hour limit on the training of the agents due to the high number of runs.}
This number of independent trials significantly surpasses the typical 3-10 runs per method used in previous policy optimization works \citep{TRPO,PPO}, motivating different results compared to the published baselines {\lmarza{Here maybe we should say that we use a penalty in the reward function. Hence, the results are not directly comparable with the original baseline...}}. Considering the computational resources used for our experiments, Appendix \ref{app:env_impact} also addresses the environmental impact. % and our strategy to offset estimated CO$_2$ emissions.

\subsection{Empirical Evaluation}
%\emarche{TODO: Experiments with varying parameters for \ourmethod} \\
\textbf{Performance of $\varepsilon$-TRPO and $\varepsilon$-PPO.} Figure \ref{fig:base_results} shows that TRPO and PPO enhanced with our \ourmethod~improve sample efficiency and allow agents to better adhere to the behavioral preferences.
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/results_base.png}
    \vspace{-5pt}
    \caption{Comparison of $\varepsilon$-PPO, $\varepsilon$-TRPO, PPO and TRPO in four different environments. Each column (i.e., each task) shows the average reward and cost during the training.}
    \label{fig:base_results}
\end{figure}
In Hopper and HalfCheetah, both TRPO and PPO achieve substantially higher returns compared to their \ourmethod\;version; a result that could be easily misunderstood. In fact, this is related to the nature of the task, where the reward is directly proportional to the agents' velocities.\footnote{Notably, the lower velocity limit of the Hopper task causes a linear relationship between average return and cost: the two functions grow in the same way.} For this reason, an agent that violates the behavioral preference \textit{``limit velocity under a threshold''}, achieves higher returns. This is clearly shown in the bottom row depicting the average cost, where $\varepsilon$-TRPO and $\varepsilon$-PPO resulted in notably lower cost compared to the baselines, indicating they lead the agents towards adhering to the velocity limit significantly more often than TRPO and PPO. Conversely, in the active network management task $\varepsilon$-TRPO is notably more sample efficient over TRPO, achieving the same performance in $\approx50\%$ of the training steps. $\varepsilon$-PPO also achieves both lower cost and higher return than PPO. At a high level, violating the operational constraints leads to higher penalties and inferior returns, and \ourmethod-enhanced algorithms learn how to operate the grid successfully (i.e., not violating operational constraints but suffering natural energy losses) using a fraction of the training steps of the baselines. The benefits of \ourmethod~are also confirmed in the navigation task, where violating the safety desiderata \textit{``avoid collisions''} leads to more collisions. Ultimately, achieving a higher cost (i.e., more collisions) hinders the navigation performance of the agent and leads to inferior returns. Specifically, TRPO and $\varepsilon$-TRPO converge to the same average cost. However, the higher sample efficiency of the latter through the training, in terms of learning collision avoidance behaviors more quickly, allows $\varepsilon$-TRPO to learn better navigation behaviors, outperforming TRPO in terms of average return. Moreover, $\varepsilon$-PPO significantly outperforms PPO both in terms of average cost and return.

\textbf{Performance of $\varepsilon$-TRPOLagr and $\varepsilon$-PPOLagr.} 
Lagrangian-based methods have been recently employed for encouraging behavioral preferences in policy optimization \citep{julien2022behavioralspec}. Here, we analyze the impact of \ourmethod~on these CMDP-based methods, modeling our desiderata as constraints.
\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{images/results_lag_new.png}
    \vspace{-5pt}
    \caption{Comparison of $\varepsilon$-PPOLagr, $\varepsilon$-TRPOLagr, PPOLagr and TRPOLagr in four different environments. Each column (i.e., each task) shows the average reward and cost during the training.}
    \label{fig:lag_results}
\end{figure}
Figure \ref{fig:lag_results} shows that constrained policy optimization algorithms enhanced with \ourmethod~reduce the constraint violations and, in the more complex tasks, allow agents to improve performance.
During training, both $\varepsilon$-TRPOLagr and $\varepsilon$-PPOLagr drastically reduce the amount of constraint violations in the Hopper and HalfCheetah velocity environments. We specify the fraction of training steps where agents violate their constraint in Table \ref{tab:violation_perc}.
However, at convergence, all the approaches satisfy the imposed thresholds. These results lead to a couple of interesting considerations based on the setup of interest. In safety-critical contexts where it is crucial to satisfy constraints at training time, \ourmethod~showed significant empirical benefits. On the other hand, in non-critical contexts where performance at convergence is the main evaluation metric, the naive Lagrangian methods have superior return performance. Intuitively, this relates to the fact that Lagrangian methods often violate the constraints at training time, allowing agents to explore more and thus learn higher-performing behaviors.
In the more complex, realistic scenarios, our empirical analysis leads to different considerations. 
\begin{table}[t]
\centering
\vspace{-5pt}
\caption{Average fraction of the training steps where agents violate the constraints (lower is better).}
\begin{tabular}{ccccc}
\toprule
    & \textbf{Hopper} & \textbf{HalfCheetah} & \textbf{Active Network Management} & \textbf{Navigation} \\ \midrule
\textbf{PPOLagr}                & 0.57   & 0.33        & \textbf{0.44}                      & 0.46       \\
\textbf{$\varepsilon$-PPOLagr}  & \textbf{0.04}   & \textbf{0}           & 0.59                      & \textbf{0.44}       \\\midrule
\textbf{TRPOLagr}               & 0.51   & 0.17        & \textbf{0.58}                      & 0.64       \\ 
\textbf{$\varepsilon$-TRPOLagr} & \textbf{0.25}   & \textbf{0}           & 0.79                      & \textbf{0.56}       \\
\bottomrule
\end{tabular}
\label{tab:violation_perc}
\end{table}
Specifically, in navigation, \ourmethod-based methods and the Lagrangian baselines achieve comparable results in terms of cost (i.e., constraint satisfaction). However, retraining agents on areas that are collision-prone, allowed the agents to learn policies with better navigation skills and higher performance. The benefits of retraining agents in areas of interest are further confirmed in the active network management task. In particular, the Lagrangian baselines fail to solve the problem successfully. In contrast, our empirical results suggest that retraining agents in situations where the power grid becomes unstable can ultimately lead agents to learn how to successfully operate the grid.


\textbf{Verifying Navigation Behaviors Provably.} 

\begin{figure}[b]
    \begin{minipage}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/density_nav_init.png}
        \par\vspace{15pt}
    \end{minipage}%
    \hspace{1pt}
    \begin{minipage}[b]{0.25\linewidth}
        \centering
        \includegraphics[width=\textwidth]{images/density_nav_end.png}
        \par\vspace{15pt}
    \end{minipage}%
    \hspace{10pt}
    \begin{minipage}[b]{0.3\textwidth}
        \input{sections/table}
        \par\vspace{-2pt}
    \end{minipage}
\caption{(left) Density map of the retrain areas collected in the first and last epochs of training; yellow indicates higher density. (right) Average behavioral violations percentage for policies trained with TRPO, PPO, PPOLagr, TRPOLagr, and their \ourmethod\;version.}
\label{tab:resultsFV}
\end{figure}

To further assess the benefit that \ourmethod~has over the behavioral preferences, we formally verify the policies trained for the navigation task. We consider this problem as an explanatory task for clarity since it allows us to easily visualize the retrain areas generated for \textit{``collision avoidance''} on top of the environment. Figure \ref{tab:resultsFV} on the left, shows a kernel density estimation map of the retrain areas distribution at the beginning (left) and final stages (right) of the training for the $\varepsilon$-TRPO agent. Here we can notice how the agent successfully learns to navigate the environment over time since the retrain areas are more equally distributed through the entire scenario.

Using the verification tool proposed by \citet{CountingProVe}, we aim to quantify the probability that a navigation policy violates the collision avoidance preference. 
To this end, we consider three representative retrain areas collected while training the different \ourmethod-based algorithms (depicted as red dots in Figure \ref{tab:resultsFV}). For each area, we encode the input-output relationship required by the tool (see Section \ref{sec:verification}), considering the retrain area as the precondition, and the minimum linear and angular velocities that would cause a collision as the postcondition. Broadly speaking, the FV tool checks where the trained policies do not exceed such minimum velocities (i.e., they do not collide), and returns the portion of each retrain area for which the given policy violates the postcondition (i.e., the probability of colliding in that area). 
Table \ref{tab:resultsFV} reports the probability that policies at convergence collide in the chosen retrain areas, averaged over all the runs. Overall, this additional analysis based on FV highlights that \ourmethod-enhanced algorithms better adhere to the behavioral preference, further confirming our intuitions and the merits of our approach.  

% show that although policies at convergence empirically achieve a comparable amount of collisions (see Figure \ref{fig:base_results}, \ref{fig:lag_results}, 

%thus making it difficult to state which one better respects specific desiderata, exploiting formal verification, it is possible to formally
%For each retrain area selected, we define a specific safety property (i.e., a behavioral preference in terms of \textit{collision avoidance}) setting for the precondition, the agent's input features encoded using the intervals collected online during training, while for the postcondition (i.e., the action to be avoided) the minimum linear and angular velocity allowed before a collision in that specific region\footnote{We note that thanks to the simulated environment it is possible to visualize each retrain area after its collection and thus given a specific agent's position centered in the area, compute the minimum linear and angular velocity allowed before a collision by exploiting the simulator physics engine.}. 




==> sections_old/introduction.tex <==
\section{Introduction}

% Exploration is a fundamental process in Reinforcement Learning (RL) as an agent initially lacks knowledge about the task to solve and must actively seek information to optimize its policy \citep{sutton1998introduction}. Without exploration, an agent can only exploit a limited understanding of the environment's dynamics and potential rewards, leading to inefficient or ineffective decision-making.

By balancing the trade-off between \textit{exploration} and \textit{exploitation}, a reinforcement learning (RL) agent can typically rely on a scalar reward function to learn behaviors capable of solving a task \citep{silver2021reward}. However, these functions often lead to unforeseen behaviors, making it difficult to enforce particular \textit{behavioral preferences} that we desire the system to exhibit \citep{amodei2016rewards}.  

For example, consider applying a policy optimization RL method to a robot learning how to reach random targets. Commonly, the agent is rewarded based on its distance from the goal and penalized for collisions \citep{drl_navigation1, drl_navigation2}, and a uniform restart distribution throughout the state space randomly initializes the environment at each episode. In this setup, learning good navigation behaviors while satisfying the preference (or desiderata, interchangeably) \textit{``avoid collisions''} requires many collisions around the same state. However, while the uniform restart distribution is pivotal to guarantee monotonic policy improvement  \citep{kakade2002approximately}, it naturally makes it harder for agents to experience these similar collisions over time. This potentially translates into a higher variance in the local estimate of the objective \citep{TRPO}, thus making it hard to effectively enforce the desired behavior \citep{eysenbach2018reset, jian2023generalization}.

% This is due to the inherent variability introduced by the random restart distribution that (potentially) leads to higher variance in the local estimate of the objective \citep{TRPO}. Additionally, the random restart makes it challenging for agents to experience similar collisions over time to generalize the behavior \citep{eysenbach2018reset, jian2023generalization}. Despite the drawbacks, using a uniform restart state distribution is key to guarantee monotonic policy improvement in policy optimization approaches \citep{kakade2002approximately}.  

To address such an issue, previous policy iteration and gradient approaches investigated the impact of restoring the environment to specific states to improve performance while maintaining theoretical guarantees on monotonic improvement \citep{lagoudakis2003reinforcement,gabillon2013approximate}. 
A leading example is the \textit{vine} Trust Region Policy Optimization (TRPO) algorithm \citep{TRPO}, designed to enhance exploration and reduce the variance of gradient updates. In detail, \textit{vine} restarts the agent in states visited under the current policy to generate additional rollouts from that state and reduce the policy update variance.
The authors also demonstrate how the theoretically justified procedure retains monotonic policy improvement guarantees. Crucially, despite the approximations required by the practical algorithm, TRPO \textit{vine} empirically results in superior performance over previous policy gradient methods based on uniform restart distributions. However, this method and, more generally, designing a poor restart state distribution has three critical downsides we address in our work. (i) To the best of our knowledge, policy optimization works have not considered restart distribution mechanisms geared towards improving specific behavioral preferences; (ii) sub-optimal distributions can cause approximate methods to get stuck in local optima, potentially resulting in poor agent performance \citep{kakade2002approximately, lagoudakis2003reinforcement}; (iii) \textit{vine} significantly hinders sample efficiency, requiring many additional rollouts for each policy update.

\begin{wrapfigure}{r}{0.49\textwidth}
  \begin{center}
    \vspace{-10pt}
\includegraphics[width=\linewidth]{images/eps_retrain.pdf}
      \end{center}
    \vspace{-3pt}
    \caption{Explanatory overview of \ourmethod.}
    \label{fig:overview}
    \vspace{-6pt}
\end{wrapfigure}

This paper presents \ourmethod, a novel exploration strategy designed to optimize policies, maintaining monotonic improvement guarantees while encouraging a behavioral preference. Our method, depicted in Figure \ref{fig:overview}, is inspired by human learning, where consistently repeating tasks enhances learning of a particular behavior. In detail, we exploit an $\varepsilon$ decay strategy to combine the uniform restart state distribution over the state space (blue), typical of RL algorithms, with a restart strategy over \textit{retrain areas} (green). The latter is modeled using an iterative procedure that collects and refines (i.e., creates and merges) portions of the state space where the agent violated the behavioral preference at training time. The proposed approach thus aims at retraining the agent from these areas, improving the advantage estimation of actions that violate the desiderata, according to a probability $\varepsilon$ (purple). Crucially, our decaying schedule for $\varepsilon$ allows us to maintain the same asymptotic convergence properties of the underlying RL algorithm and, along with the design of retraining areas, ensure that we avoid sub-optimal distributions. Our method also does not require additional rollouts and we demonstrate that using mixed uniform restart distributions leads, in the worst case, to the same monotonic improvement guarantees as in \citet{TRPO}.

We first empirically demonstrate the benefits of employing \ourmethod~on top of policy optimization methods (i.e., TRPO \citep{TRPO} and Proximal Policy Optimization (PPO) \citep{PPO}) over hundreds of seeds and different behavioral preferences. % that also maps in the literature to safety requirements \citep{ray2019safetygym, stooke2020lagpid}. 
We also combine \ourmethod~with the Lagrangian implementations of TRPO and PPO since they have been recently employed to enforce specific behavior \citep{julien2022behavioralspec}.  
Our evaluation considers diversified tasks ranging from simulated locomotion to optimizing power networks and robotic navigation. The results show that enhancing policy optimization methods with \ourmethod~leads to significantly higher sample efficiency and better enforce the behavioral desiderata while solving the tasks. Crucially, we note that system designers typically evaluate if agents comply with the expected behavior empirically and can not provably quantify the degree to which they adhere to the preferences. Since our theory refers to the improvement over the main reward objective, we employ a formal verification (FV) of neural networks tool to provably quantify the rate at which the agent trained for the navigation task avoids collisions in the retrain areas.\footnote{We use navigation as an explanatory task for clarity since it allows us to visualize retrain areas.} Finally, the realistic Unity environment employed in the robotic navigation task
enables the transfer of policies trained in simulation on ROS-enabled
platforms. Hence, we show the effectiveness of \ourmethod\;in realistic unsafe navigation scenarios.



==> sections_old/method.tex <==
\section{Policy Optimization via \ourmethod}
\label{sec:method_theory}

We introduce \ourmethod~to retrain an RL agent from regions of the state space where it previously violated a behavioral preference. Our goal is to encourage a policy to follow such desiderata while improving performance and sample efficiency. To this end, \ourmethod~introduces a \textit{mixed restart distribution}, combining the typical uniform restart distribution $\rho$ over the entire state space $\mathcal{S}$, with another uniform restart distribution $\overline{\rho}:\overline{\mathcal{S}} \to [0, 1]$ defined over a retrain area. Such an area is a subset of the original state space $\overline{\mathcal{S}} \subseteq \mathcal{S}$ and is defined using an iterative procedure that collects and (potentially) refines parts of $\mathcal{S}$ where the agent violated the behavioral preference during training. Crucially, such a procedure is orthogonal to policy optimization literature, and can potentially be applied to any RL algorithm. 
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.9\linewidth]{images/overview.pdf}
%     \caption{Explanatory overview of \ourmethod.}
%     \vspace{-10pt}
%     \label{fig:overview}
% \end{figure}
\subsection{\ourmethod\;overview}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/overview2.pdf}
    \caption{Explanatory overview of \ourmethod.}
   \vspace{-0.6cm}
    \label{fig:overview}
\end{figure}
We provide a detailed discussion of the procedure in Algorithm 1, considering a generic RL training procedure as a baseline, while Figure \ref{fig:overview} provides a schematic representation of \ourmethod. 

In detail, on the left of Figure \ref{fig:overview}, we show the typical training loop of an RL agent, on the right the iterative procedure for generating the retrain areas, and in the middle the mixed restart distribution, respectively. %These components are discussed in Algorithm \ref{alg:eps_retrain}, which highlights the pseudocode for \ourmethod~considering a generic RL training procedure as a baseline.
%Similarly to common $\varepsilon$-greedy policy exploration strategies, \ourmethod~employs a linear decay for the mixed restarting distribution (line 1). 
At the beginning of each episode, the initial state of the environment is either randomly sampled from the whole state space $\mathcal{S}$ with probability $1-\varepsilon$, or randomly sampled from a retrain area with probability $\varepsilon$. If the realized sample is from a retrain area, this means the environment resets to a configuration where the agent violated the behavioral preference in the previous trajectories. Similarly to common $\varepsilon$-greedy policy exploration strategies, \ourmethod~employs a linear decay for the mixed restarting distribution (line 1).

Upon each violation of behavioral desiderata, a retrain area is created and collected into a queue $\mathcal{B}$ that is initially empty; it is possible to set a maximum size for $\mathcal{B}$ to limit the horizon over which retraining an agent (lines 2-10).
To detect the interactions where the agent violates the desiderata, we use an indicator cost signal as in the safe RL literature \citep{altman1999cmdp, ray2019safetygym, ji2023omnisafe}.
During the execution of the chosen RL algorithm, the iterative procedure for collecting and refining the retrain areas begins upon receiving a positive cost (lines 11-13). We start by collecting an initial area---a small portion of the space surrounding the state that led to a violation (i.e., a bubble around the state). This is achieved by encoding each feature of the agent's state as an interval with fixed size $\phi$ (line 14). Figure \ref{fig:overview_crop} shows an explanatory example in the navigation scenario, where collision avoidance is our desired preference. 
\begin{algorithm}[h]
\caption{\ourmethod}\label{alg:eps_retrain}
\begin{algorithmic}[1]
\Require \textit{bubble} size $\phi$ for initializing a retrain area, \textit{similarity} value $\beta$ to merge similar areas, \textit{decay}, \textit{initial}, and \textit{minimum} values for the $\varepsilon$ scaling.

\State $\varepsilon\_decay  \gets (min\_\varepsilon -1.0)/(decay\cdot(epochs    \cdot steps\_per\_epoch))$;
\State $\mathcal{B} \gets \emptyset$ \Comment{Initialize buffer of retrain areas}
\For{each episode}
\If{$random(0,1) < \varepsilon \wedge \mathcal{B} \neq \emptyset$}
    \State $r \gets \texttt{sample\_retrain\_area}(\mathcal{B})$ \Comment{randomly sample a retrain area}
    \State $s_0 \gets \texttt{sample\_state}(r)$ \Comment{randomly sample a state from the retrain area}
    \State $\varepsilon \gets  \max(\varepsilon\_decay\cdot(epoch)*steps\_per\_epoch + 1.0,\; min\_\varepsilon)$
\Else
    \State $s_0 \gets \rho(\mathcal{S})$ \Comment{select the starting state using the original restart distribution}
\EndIf
\While{episode is not done}
    \State Execute the typical training loop of the chosen RL algorithm for each step $t$.
    \If{$s_{t}$ is unsafe (i.e., cost $> 0$)}
         \State $r \gets \texttt{generate\_retrain\_area}(s_{t-1}, \phi)$
         \If{$\exists\; r'\ \in\mathcal{B}$ \text{that is} $\beta$-similar to $r$}
            \State $r \gets \texttt{area\_refinement}(r,r')$
         \EndIf
         \State $\mathcal{B} \gets \mathcal{B} \cup r$
    \EndIf    
\EndWhile
\EndFor
\end{algorithmic}
\end{algorithm}
By leveraging commonly available task knowledge (in this case, the robot sensors' precision), we encode a bubble of size $\phi$ around the state that led to the collision. Our idea is that retraining an agent from these slightly different situations could improve performance. 

\begin{wrapfigure}{l}{0.49\textwidth}
  \begin{center}
    \vspace{-10pt}
\includegraphics[width=\linewidth]{images/retrain_area.png}
      \end{center}
    \caption{Creating a retrain area for a navigation task. (left) The agent collides with an obstacle, receiving a positive cost. (right) A retrain area is created from the state that led to the collision.}
    \label{fig:overview_crop}
    \vspace{-5pt}
\end{wrapfigure}
After modeling the new retrain area, the refinement procedure starts (lines 15-17). We define a similarity rule to decide whether to merge two retrain areas, indicating they model a similar violation. Specifically, if two retrain areas are within a distance $\beta$ (a hyper-parameter of \ourmethod), they are combined by taking the minimum lower bound and the maximum upper bound of the two for each input feature's interval. The refinement offers two advantages: (i) it allows us to maintain a reasonable size for $\mathcal{B}$. (ii) It clusters similar behavioral violations within the same retrain area, guaranteeing a uniform sampling over different behavioral violations. Finally, the new or refined area is inserted into $\mathcal{B}$ and could then be used to retrain the agent (line 18).

%After the unsafe regions buffer begins to be populated and a desired $\varepsilon$ decay is fixed, our approach begins to mix the initial state distributions $\rho$ and $\overline{\rho}$, as shown in the right part of Fig. \ref{fig:overview}. 
%Specifically, $\varepsilon$ times that $\overline{\rho}$ is selected, one of the unsafe regions from the buffer is randomly sampled (highlighted with the red dots in the red subspace $\overline{\rho}$ of Fig. \ref{fig:overview}). Operating under the assumption that everything within that region is potentially unsafe, we then randomly pick an initial state $s_0$ to initiate the new trajectory. It is worth noting that this assumption is not overly restrictive, as with a high probability, considering a state surround of reasonable size at the time of the unsafe interaction in the environment, unlikely we will sample a completely safe state. Even in the rare scenario where this might occur, the correctness of the method remains unaffected, given that $\mathcal{\overline{S}} \subseteq \mathcal{S}$. 

\subsection{Limitations and Assumptions}
\ourmethod~shares the same downside as most RL algorithms, which is that it requires the system to be restored to particular states, which is typically only possible in simulation.
Our algorithm also makes several assumptions, though we believe they do not hinder the applicability of our method. In particular, we assume having access to an additional indicator cost signal from the environment. Such a signal is widely adopted in the safe RL literature where system designers assume having access to a cost function that deems a state-action pair as safe or unsafe \citep{altman1999cmdp, ray2019safetygym, ji2023omnisafe}. Moreover, we assume the area surrounding a collision state is also prone to violations of the desiderata. When such an assumption does not hold (e.g., in highly non-linear systems such as power grids), there are two possible considerations: (i) we could use the exact feature values to determine a retrain area, instead of intervals of size $\phi$. (ii) The agent simply restarts from a random state within the retrain area, which does not hinder the overall training process. 


\subsection{Monotonic Improvement Guarantees}

In this section, we derive a bound on the monotonic policy improvement for \ourmethod~enhanced algorithms employing a mixture of uniform restart distributions. Notably, our result motivates both the design of our method as well as its superior performance (Section \ref{sec:experiments}).\footnote{We note the theoretically justified procedure motivating the policy improvement bound \citep{TRPO} does not hold for most practical policy optimization algorithms such as TRPO and PPO.}
For the sake of clarity, we first recall the definition of \textit{$\alpha$-coupled policies} and the related lemma introduced to derive the bound in case of a single uniform restart distribution over $\mathcal{S}$. First, Definition \ref{def:coupling} couples two policies that behave in the same way (i.e., given a state, they pick the same action) with probability $\geq 1-\alpha$, and Lemma \ref{lem:bound} bounds the gap between policy advantages satisfying such policies.
\begin{definition}[$\alpha$-coupled policies \citep{TRPO}]\label{def:coupling}
    We say that $\pi$ and $\pi'$ are two $\alpha$-coupled policies if $\forall s \in\mathcal{S}$, we can define a joint distribution $(a, a') \vert s$ such that $P(a \neq a'\vert s) \leq \alpha$.
\end{definition}
\begin{lemma}[\citet{TRPO}] \label{lemma1}
    Given two $\alpha$-coupled policies, $\pi$ and $\pi'$, we have that:
    \begin{equation}
        \left\vert \mathbb{E}_{s_t\sim\pi'}[\Tilde{A}(s_t)] - \mathbb{E}_{s_t\sim\pi}[\Tilde{A}(s_t)]\right\vert \leq 4\alpha(1-(1-\alpha)^t)\max_{s,a}\vert A_\pi(s,a)\vert.
    \end{equation}
    It follows that:
        $\vert \psi(\pi') - L_\pi(\pi')\vert$ $\leq \frac{4\alpha^2 \gamma k}{(1-\gamma)^2}$ with $k= \max\limits_{s,a}\vert A_\pi(s,a) \vert$.
\label{lem:bound}
\end{lemma}

However, Lemma \ref{lem:bound} only considers the case where a uniform restart distribution over $\mathcal{S}$ is used. We extend such result to the mixture of restarting distributions used by \ourmethod, starting by defining the expected discounted return of a new policy $\pi'$ over the current one $\pi$ as:

\begin{equation} \label{eq1_new}
     \overline{\psi}(\pi') = (1-\varepsilon)\Bigg[\psi(\pi) + \mathbb{E}_{ \substack{ \tau \sim \pi' \\ s_0 \sim \rho}} \Big[\sum_{t=0}^\infty \gamma^t \Tilde{A}(s_t) \Big]\Bigg]+(\varepsilon)\Bigg[\psi(\pi) + \mathbb{E}_{ \substack{ \tau \sim \pi' \\ s_0 \sim \overline{\rho}}} \Big[\sum_{t=0}^\infty \gamma^t \Tilde{A}(s_t) \Big]\Bigg]
\end{equation}

For the surrogate loss (see Equation \ref{eq2}), we obtain its local approximation:

\begin{equation} \label{eq2_new}
\overline{L}_\pi(\pi') = (1-\varepsilon)\Bigg[\psi(\pi) + \mathbb{E}_{\substack{ \tau \sim \pi \\ s_0 \sim \rho }} \Big[\sum_{t=0}^\infty \gamma^t \Tilde{A}(s_t) \Big]\Bigg] + (\varepsilon)\Bigg[\psi(\pi) + \mathbb{E}_{\substack{ \tau \sim \pi \\ s_0 \sim \overline{\rho}}} \Big[\sum_{t=0}^\infty \gamma^t \Tilde{A}(s_t) \Big]\Bigg]
\end{equation}

We thus extend Lemma \ref{lem:bound} to provide an upper bound on the distance between $\overline{\psi}(\pi')$ and  $\overline{L}_\pi(\pi')$ under the mixed restart state distribution of \ourmethod. 

\begin{lemma} \label{ourlemma}
    Considering a mixed restart distribution using \ourmethod, the difference is
    $\vert \overline{\psi}(\pi') - \overline{L}_\pi(\pi')\vert \leq \frac{4\alpha^2 \gamma}{(1-\gamma)^2}\Big[k(1-\varepsilon)+ k'\varepsilon\Big] \leq \frac{4\alpha^2 \gamma k}{(1-\gamma)^2} $ with $k' \leq k= \max\limits_{s,a}\vert A_\pi(s,a) \vert$.
\label{lem:epsbound}
\end{lemma}

Appendix \ref{app:proof} provides a formal proof. The correctness of our result stems from the following facts: (i) $\alpha$-coupled policies are coupled over the entire $\mathcal{S}$, ensuring that policies are coupled even when combining $\rho$ and $\overline{\rho}$. (ii) $k$ is defined as the maximum over all $s \in \mathcal{S} \supseteq \mathcal{\overline{S}}$ and, as such, $k \geq k'$. In more detail, Lemma \ref{ourlemma} shows that enforcing the agent to start from retraining areas can help in narrowing the gap between the $\psi(\pi')$ and the local approximation $L_\pi(\pi')$. In fact, when $k=k'$, the difference reduces to the original case of Lemma \ref{lem:bound}. In contrast, $k' < k$ indicates that the trajectories starting from a retrain area do not result in an improved advantage. This provides a more precise understanding of the portion of the state space where the policy yields the best advantage. Broadly speaking, it has the effect of incorporating prior knowledge about the advantages.

Finally, exploiting the relationship between the total variation divergence and the KL divergence \citep{pollard2000asymptopia}, we derive the following corollary on the monotonic improvement guarantee under \ourmethod~-based methods.
\begin{corollary}
    Let $\rho$ and $\overline{\rho}$ be two different restart distributions. Combining $\rho$ and $\overline{\rho}$ during the training as in \ourmethod, and by setting $\alpha$ as Eq. \ref{eq:boundSchulman}, the bound on the monotonic improvement for the policy update %derived in \citep{TRPO} 
    $\overline{\psi}(\pi') \geq \overline{L}_\pi(\pi') - CD^{max}_{KL}(\pi, \pi')$ with $C=\frac{4k\gamma}{1-\gamma^2} $ 
    is still guaranteed.
\end{corollary}

The result naturally follows from Lemma \ref{ourlemma} and the derivation of \citet{TRPO}.

==> sections_old/method_new.tex <==
\section{Policy Optimization via \ourmethod}
\label{sec:method_theory}
We introduce \ourmethod~to restart an agent from regions of the state space where it previously violated a behavioral preference. Our goal is to encourage a policy to follow the desiderata while improving performance and sample efficiency. To this end, \ourmethod~collects retrain areas---subsets of the state space $\overline{\mathcal{S}} \subseteq \mathcal{S}$ defined using an iterative procedure that merges parts of $\mathcal{S}$ where the agent violated the preference during training. We then introduce a \textit{mixed restart distribution}, combining the typical uniform restart distribution $\rho$ over the entire state space $\mathcal{S}$, with another uniform restart distribution $\overline{\rho}:\overline{\mathcal{S}} \to [0, 1]$ that considers retrain areas. Crucially, such a procedure is simple to implement and can potentially be applied to any policy optimization RL algorithm. 

\begin{wrapfigure}{l}{0.45\textwidth}
  \begin{center}
  \vspace{-12pt}
\includegraphics[width=0.85\linewidth]{images/retrain_area.png}
      \end{center}
    \vspace{-6pt}
    \caption{(left) The agent collides with an obstacle, receiving a positive cost. (right) A retrain area is created from that state.}
    \label{fig:overview_crop}
    \vspace{-9pt}
\end{wrapfigure}
In the RL training loop, the iterative procedure for collecting and merging retrain areas begins upon receiving a positive cost. 
We use an indicator cost signal (as in the safe RL literature \citep{garcia2015safety}) to detect the interactions where the agent violates the desiderata. Upon each violation, a retrain area is created and collected into a buffer $\overline{\mathcal{S}}$ that is initially empty.\footnote{Note that it is possible to set a maximum size for $\overline{\mathcal{S}}$ to limit the horizon over which retraining an agent.} Such an area is a portion of the space surrounding the state that led to a violation, created by encoding each feature of the agent's state as an interval with fixed size $\omega$ (i.e., a ``bubble'' around the state). 
Figure \ref{fig:overview_crop} shows an explanatory example in the navigation task, where collision avoidance is our desiderata. By leveraging commonly available information (in this case, the sensors' precision), we encode a bubble of size $\omega$ around the state that led to the collision. The idea is that retraining an agent from these slightly different, collision-prone situations could improve performance. 
After modeling the new retrain area, a refinement procedure starts. In detail, we define a similarity rule to decide whether to merge two retrain areas, indicating they model a similar violation. Specifically, if two retrain areas are within a distance $\beta$ (a hyper-parameter of \ourmethod), they are combined by taking the minimum lower and maximum upper bounds of the two for each input feature's interval. The refinement offers two advantages: (i) it allows us to maintain a reasonable size for $\overline{\mathcal{S}}$, and (ii) it clusters similar behavioral violations within the same retrain area, guaranteeing a uniform sampling over different violations. The new or refined area is then inserted into $\overline{\mathcal{S}}$ and can be used to retrain the agent.
Finally, before starting the next episode, the new initial state of the environment is either randomly sampled from the whole state space $\mathcal{S}$ with probability $1-\varepsilon$, or randomly sampled from a retrain area with probability $\varepsilon$. If the realized sample is from a retrain area, this means the environment resets to a configuration where the agent violated the behavioral preference in the previous trajectories. Crucially, \ourmethod~employs a linear decay for the mixed restarting distribution, avoiding the problem of getting stuck in suboptimal restart distributions. 

We refer to Appendix \ref{app:eps-retrain} for an explanatory example of the generation and refinement of retrain areas and for the detailed pseudocode of our method. 

\section{Monotonic Improvement Guarantees}

%In this section, we derive a bound on the monotonic policy improvement for \ourmethod~enhanced algorithms employing a mixture of uniform restart distributions. Notably, our result motivates both the design of our method as well as its superior performance (Section \ref{sec:experiments}).
In this section, we theoretically derive a bound on the monotonic policy improvement for approaches that employ a mixture of uniform restart distributions, similar to \ourmethod. We show that the original bound on monotonic policy improvement presented by \citet{TRPO} still holds and, in some cases, can be tighter. Notably, our result motivates both the design of our method as well as its superior performance (Section \ref{sec:experiments}).
For the sake of clarity, we first recall the definition of \textit{$\alpha$-coupled policies} and the related lemma introduced to derive the bound in case of a single uniform restart distribution over $\mathcal{S}$. First, Definition \ref{def:coupling} couples two policies that behave in the same way (i.e., given a state, they pick the same action) with probability $\geq 1-\alpha$, and Lemma \ref{lem:bound} bounds the gap between policy advantages satisfying such policies.
\begin{definition}[$\alpha$-coupled policies \citet{TRPO}]\label{def:coupling}
    We say that $\pi$ and $\pi'$ are two $\alpha$-coupled policies if $\forall s \in\mathcal{S}$, we can define a joint distribution $(a, a') \vert s$ such that $P(a \neq a'\vert s) \leq \alpha$.
\end{definition}
\begin{lemma}[\citet{TRPO}] \label{lemma1}
    Given two $\alpha$-coupled policies, $\pi$ and $\pi'$, we have that: $\left\vert \mathbb{E}_{s_t\sim\pi'}[\Tilde{A}(s_t)] - \mathbb{E}_{s_t\sim\pi}[\Tilde{A}(s_t)]\right\vert \leq 4\alpha(1-(1-\alpha)^t)\max_{s,a}\vert A_\pi(s,a)\vert$.
    It follows that: $\vert \psi(\pi') - L_\pi(\pi')\vert$ $\leq \frac{4\alpha^2 \gamma k}{(1-\gamma)^2}$ with $k= \max\limits_{s,a}\vert A_\pi(s,a) \vert$.
\label{lem:bound}
\end{lemma}

Lemma \ref{lem:bound}, however, only considers the case where a uniform restart distribution over $\mathcal{S}$ is used. We extend such result to the mixture of restarting distributions used by \ourmethod~(right side of Equation \ref{eq:mixture_return}, where $s_0\sim\overline{\rho}$), starting by defining the expected discounted return of a new policy $\pi'$ over the current $\pi$ as:
\begin{equation}
    \footnotesize
     \overline{\psi}(\pi') = (1-\varepsilon)\Bigg[\psi(\pi) + \mathbb{E}_{ \substack{ \tau \sim \pi' \\ s_0 \sim \rho}} \Big[\sum_{t=0}^\infty \gamma^t \Tilde{A}(s_t) \Big]\Bigg]+(\varepsilon)\Bigg[\psi(\pi) + \mathbb{E}_{ \substack{ \tau \sim \pi' \\ s_0 \sim \overline{\rho}}} \Big[\sum_{t=0}^\infty \gamma^t \Tilde{A}(s_t) \Big]\Bigg].
\label{eq:mixture_return}
\end{equation}

For the surrogate loss (see Equation \ref{eq2}), we obtain its local approximation:

\begin{equation} \label{eq2_new}
\footnotesize
\overline{L}_\pi(\pi') = (1-\varepsilon)\Bigg[\psi(\pi) + \mathbb{E}_{\substack{ \tau \sim \pi \\ s_0 \sim \rho }} \Big[\sum_{t=0}^\infty \gamma^t \Tilde{A}(s_t) \Big]\Bigg] + (\varepsilon)\Bigg[\psi(\pi) + \mathbb{E}_{\substack{ \tau \sim \pi \\ s_0 \sim \overline{\rho}}} \Big[\sum_{t=0}^\infty \gamma^t \Tilde{A}(s_t) \Big]\Bigg].
\end{equation}

We thus extend Lemma \ref{lem:bound} to provide an upper bound on the distance between $\overline{\psi}(\pi')$ and  $\overline{L}_\pi(\pi')$ under the mixed restart state distribution of \ourmethod. 

\begin{lemma} \label{ourlemma}
    Considering a mixed restart distribution over $\rho$ and $\overline{\rho}$ using \ourmethod, it holds that
    $$\vert \overline{\psi}(\pi') - \overline{L}_\pi(\pi')\vert \leq \frac{4\alpha^2 \gamma}{(1-\gamma)^2}\Big[k(1-\varepsilon)+ k'\varepsilon\Big] \leq \frac{4\alpha^2 \gamma k}{(1-\gamma)^2} $$ with $k'= \max\limits_{\substack{
    s_0 \sim \overline{\rho}\\ \tau \sim \pi'}}\vert A_{\pi'}(s,a) \vert \leq k= \max\limits_{\substack{s_0 \sim \rho \\ \tau \sim \pi'}}\vert A_{\pi'}(s,a) \vert$, $\varepsilon \in [0,1]$.
\label{lem:epsbound}
\end{lemma}
\textit{Proof.} Full proof of Lemma \ref{lem:epsbound} is presented in Appendix \ref{app:proof}. $\quad\hfill \ensuremath{\Box}$ 


%The correctness of our result stems from the following facts: (i) $\alpha$-coupled policies are coupled over the entire $\mathcal{S}$, ensuring that policies are coupled even when combining $\rho$ and $\overline{\rho}$, and (ii) $k$ is defined as the maximum over all $(s, a) \in (\mathcal{S} \supseteq \mathcal{\overline{\mathcal{S}}}, \mathcal{A})$ and, as such, $k \geq k'$. In more detail, Lemma \ref{ourlemma} shows that enforcing the agent to start from retraining areas can help in narrowing the gap between the $\psi(\pi')$ and the local approximation $L_\pi(\pi')$. In fact, when $k=k'$, the difference reduces to the original case of Lemma \ref{lem:bound}. 
%In contrast, when $k' < k$, the trajectories induced by $\overline{\rho}$ are not optimal since agents are penalized for violating the preference.
%Thus, the agent gains a more precise understanding of the portion of the state space where the policy does not yield the maximum possible advantage. 
Finally, by exploiting the relationship between the total variation divergence and the KL divergence \citep{pollard2000asymptopia}, we derive the following corollary on the monotonic improvement guarantee under \ourmethod-based methods.
\begin{corollary}
    Let $\rho$ and $\overline{\rho}$ be two different restart distributions. Combining $\rho$ and $\overline{\rho}$ during the training as in \ourmethod, and by setting $\alpha=D_{KL}^{max}(\pi, \pi')$, the bound on the monotonic improvement for the policy update %derived in \citep{TRPO} 
    $\overline{\psi}(\pi') \geq \overline{L}_\pi(\pi') - CD^{max}_{KL}(\pi, \pi')$ with $C=\frac{4k\gamma}{1-\gamma^2} $ 
    is still guaranteed.
\end{corollary}

The result naturally follows from Lemma \ref{ourlemma} and the derivation of \citet{TRPO}.%\footnote{We note the theoretically justified procedure motivating the policy improvement bound \citep{TRPO} does not hold for most practical deep RL policy optimization algorithms.}


\section{Limitations and Assumptions of \ourmethod}

Our algorithm requires a simulator to train the agent and the possibility of resetting the system to specific states. We believe the latter requirement is reasonable, and it has been also considered by previous work \citep{TRPO}.
%\ourmethod~ also relies on several assumptions, though we believe they do not hinder its applicability. In particular, we assume having access to an additional indicator cost signal from the environment. 
In \ourmethod~, we assume having access to an additional indicator cost signal from the environment. Such a signal is widely adopted in the safe RL literature, where system designers assume having access to a cost function that deems a state-action pair as safe or unsafe \citep{altman1999cmdp, ray2019safetygym, ji2023omnisafe}. Finally, we assume the area surrounding a collision state is also prone to violations of the desiderata. When such an assumption does not hold (e.g., in highly non-linear systems such as power grids), we could use the exact feature values to determine a retrain area instead of intervals of size $\omega$.

==> sections_old/preliminaries.tex <==
\section{Preliminaries and Related Work}\label{preliminaries}

%\subsection{Problem Formulation}
We consider problems defined as Markov decision processes (MDPs), modeled as a tuple $(\mathcal{S}, \mathcal{A}, \mathcal{P}, \rho, R, \gamma)$; $\mathcal{S}$ and $\mathcal{A}$ are the finite sets of states and actions, respectively, $\mathcal{P}:\mathcal{S \times \mathcal{A} \times \mathcal{S}} \to [0, 1]$ is the state transition probability distribution, $\rho: \mathcal{S}\to [0, 1]$ is the initial uniform state distribution, $R: \mathcal{S}\times\mathcal{A} \to \mathbb{R}$ is a reward function, and $\gamma\in [0,1)$ is the discount factor. In policy optimization algorithms, agents learn a parameterized stochastic policy $\pi:\mathcal{S} \times \mathcal{A} \to [0,1]$, modeling the probability to take an action $a_t \in \mathcal{A}$ in a state $s_t \in \mathcal{S}$ at a certain step $t$. The goal is to find the parameters that maximize the expected discounted reward $\psi(\pi) = \mathbb{E}_{\tau\sim\pi} [\sum_{t=0}^\infty \gamma^t R(s_t, a_t)]$,
where $\tau:= (s_0, a_0, s_1, a_1, \dots)$ is a trajectory with $s_0 \sim \rho(s_0)$, $a_t \sim \pi(a_t \vert s_t)$, $s_{t+1} \sim \mathcal{P}(s_{t+1} \vert s_t, a_t)$. 

We also define state and action value functions $V_\pi$ and $Q_\pi$ modeling the expected discount return starting from the state $s_t$ (and action $a_t$ for $Q_\pi$) and following the policy $\pi$ thereafter as: $V_\pi(s_t) = \mathbb{E}_{a_t, s_{t+1}, a_{t+1},\dots}[ \sum_{i=0}^\infty \gamma^i R(s_{t+i}, a_{t+i})]$ and $Q_\pi(s_t, a_t) = \mathbb{E}_{s_{t+1}, a_{t+1},\dots}[ \sum_{i=0}^\infty \gamma^i R(s_{t+i}, a_{t+i})]$.
Moreover, given the current state and action, we can measure how much better or worse the agent performs compared to its expected performance---the advantage function: 
$A_\pi(s,a) = Q_\pi(s,a) - V_\pi(s) = \mathbb{E}_{s' \sim \mathcal{P}(s' \vert s,a)}[R(s,a)+ \gamma V_\pi(s')-V_\pi(s)]$. %Similarly, the state-action value function is defined as:
%$$Q_\pi(s_t, a_t) = \mathbb{E}_{s_{t+1}, a_{t+1},\dots}\Bigg[ \sum_{k=0}^\infty \gamma^k R(s_{t+k}, a_{t+k}) \Bigg] $$
To derive a bound on the policy improvement, \citet{TRPO} also define the expected advantage of a new policy $\pi'$ over the old $\pi$, and relate the expected discounted return of $\pi'$ to $\pi$: $\Tilde{A}(s) = \mathbb{E}_{a \sim \pi'(\cdot \vert s)}[A_\pi(s,a)]$, and $ \psi(\pi') = \psi(\pi) + \mathbb{E}_{\tau \sim \pi'}[\sum_{t=0}^\infty \gamma^t A_{\pi}(s_t, a_t)]$. In practice, the dependency on trajectories induced by $\pi'$ makes the above equation hard to optimize. To address this, \citet{TRPO} introduce a surrogate local approximation $L_\pi(\pi')$ to $\psi(\pi')$, using the state distribution over the current policy $\pi$ rather than $\pi'$:
\begin{equation}
    \footnotesize
    L_\pi(\pi') = \psi(\pi) + \sum_s \rho_\pi(s) \sum_a \pi'(a \vert s) A_\pi(s,a) = \psi(\pi) + \mathbb{E}_{\tau \sim \pi} \Bigg[\sum_{t=0}^\infty \gamma^t \Tilde{A}(s_t) \Bigg]. 
\label{eq2}
\end{equation}
With the above intuitions, it is possible to derive an upper bound on the absolute difference between $\vert \psi(\pi') - L_\pi(\pi')\vert \leq \frac{4\alpha^2 \gamma k}{(1-\gamma)^2}$, with $k= \max\limits_{s,a}\vert A_\pi(s,a) \vert$. Finally, by setting $\alpha = D^{\text{max}}_{KL}(\pi, \pi') = \max\limits_{s} D_{KL}(\pi(\cdot \vert s) \;\vert \vert\; \pi'(\cdot \vert s))$ and employing the relationship between the total variation (TV) divergence and the Kullback–Leibler (KL) divergence $D_{TV}(p\vert\vert q)^2 \leq D_{KL}(p\vert\vert q)$ \citep{pollard2000asymptopia}, \citet{TRPO} derive and prove the following lower bound on the policy improvement:  $\psi(\pi') \geq L_\pi(\pi') - CD^{\text{max}}_{KL}(\pi, \pi')$, with $C=\frac{4k\gamma}{1-\gamma^2}$.
% \begin{equation} 
%     \psi(\pi') \geq L_\pi(\pi') - CD^{\text{max}}_{KL}(\pi, \pi'), \quad \text{with } C=\frac{4k\gamma}{1-\gamma^2}.
% \label{eq:boundSchulman}
% \end{equation}

\subsection{Constrained MDP}
Constrained optimization has been recently employed to encourage a behavioral preference, or a safety specification \citep{ray2019safetygym, stooke2020lagpid, julien2022behavioralspec}. To this end, the classical MDP extends to a constrained MDP (CMDP) considering an additional set of $\mathcal{C} := \{C_i\}_{i\in n}$ indicator cost functions and $\mathbf{l} \in \mathbb{R}^n$ hard-coded thresholds for the constraints \citep{altman1999cmdp}. The goal of constrained RL algorithms is to maximize the expected reward while limiting the accumulation of costs under the thresholds. To this end, policy optimization algorithms typically employ the Lagrangian to transform the problem into an unconstrained one that is easy to implement over existing algorithms \citep{nocedal2006book}. 

Consider the case of a single constraint characterized by a cost function $C: \mathcal{S}\times\mathcal{A} \to \{0, 1\}$, for which we can define the expected cost function $\psi_C(\pi) := \mathbb{E}_{\tau\sim\pi}\left[\sum_{t=0}^\infty \gamma^t C(s_t, a_t) \right],$ as well as a cost threshold $l$.
The Lagrangian applies a differentiable penalty $\mathcal{L}_{\mathcal{C}}(\lambda)  = -\lambda\left(\psi_C(\pi) - l\right)$ to the policy optimization objective, where $\lambda$ is the so-called \textit{Lagrangian multiplier}. These algorithms thus take an additional gradient descent step in $\lambda$: $\nabla_\lambda \mathcal{L}_{\mathcal{C}}(\lambda) = l - \psi_C(\pi)$. The multiplier is forced to be $\geq 0$ as it acts as a penalty when the constraint is not satisfied (\textit{i.e.}, $\lambda$ increases) while decreasing to $0$ and removing any penalty when the constraint holds.
However, choosing arbitrary small values for the threshold potentially causes a detrimental trade-off between the main task and cost objectives, ultimately leading to policies that fail to solve the problem they are trained for. Moreover, the cost metric employed in the safety evaluation is purely empirical and does not provide any provable guarantees on the actual adherence to behavioral preferences. To address such an issue, employing formal verification of neural networks becomes of pivotal importance.

\subsection{Formal Verification of Neural Networks}
\label{sec:verification}
A reachability-based FV for neural networks tool takes as input a tuple $\mathcal{T} = \langle \mathcal{F}, \mathcal{X}, \mathcal{Y}\rangle$, where $\mathcal{F}$ is the trained policy (i.e., the neural network), and $\langle \mathcal{X}, \mathcal{Y}\rangle$ encodes a behavioral preference in terms of input-output relationships \citep{LiuSurvey}. 
Specifically, $\mathcal{X}$ is a precondition defined on the portion of the state space we are interested in, and $\mathcal{Y}$ models the postcondition specifying the desiderata. %Due to the continuous nature of DNNs, $\mathcal{X}$ and $\mathcal{Y}$ are typically expressed using convex geometries. %, for instance, a cartesian product of hyperrectangles or halfspaces. 
\begin{wrapfigure}{r}{0.49\textwidth}
  \begin{center}
     \vspace{-5mm}
    \includegraphics[width=\linewidth]{images/FV.png}
      \end{center}
    \vspace{-5pt}
    \caption{Overview of FV for neural networks.}
    \label{fig:overviewFV}
    \vspace{-5mm}
\end{wrapfigure}
An FV tool propagates intervals $\mathcal{X}$ through $\mathcal{F}$ and performs a layer-by-layer reachability analysis to compute the output reachable set $\mathcal{R}(\mathcal{X}, \mathcal{F})$. The tool then checks if $\mathcal{R}(\mathcal{X}, \mathcal{F}) \subseteq \mathcal{Y}$, meaning that the agent satisfies the preference for all the states in $\mathcal{X}$.
Figure \ref{fig:overviewFV} shows a simplified overview of the verification process, which checks if (at least) one violation of the behavioral preference exists in $\mathcal{X}$. Due to over-approximation errors introduced by the propagations, FV tools iteratively split $\mathcal{X}$ into sub-domains $\mathcal{X}_i$ \citep{reluval} (the first two blocks). When the output reachable set $\mathcal{R}(\mathcal{X}_i, \mathcal{F})$ is not included in $\mathcal{Y}$ (the second to last block), the iterative procedure ends---the behavioral preference is violated if at least one portion of the domain $\mathcal{X}$ falls within this scenario. As a natural extension of the FV problem, recent works \citet{CountingProVe,patching} propose to enumerate all the portions of $\mathcal{X}$ violating the desiderata, thus provably quantifying the rate at which agents satisfy the input-output relationships. In this work, we rely on the tool proposed by \cite{CountingProVe} to quantify the degree to which agents adhere to behavioral preferences in the robotic navigation task. %We note that reachability-based methods have also been considered as a way to ``repair'' neural networks in the context of safety \citep{patching}. Although effective, these methods are prone to catastrophic forgetting and do not scale to our setups due to the NP-complete nature of FV \citep{Reluplex}. 

==> sections_old/table.tex <==
\tiny
\begin{tabular}{@{\extracolsep{-5pt}}ccccc}
 \toprule &\multicolumn{3}{c}{\textbf{Retrain areas (1, 2, 3)}} 
\\
\midrule 
 \makecell[l]{$\varepsilon $-PPO\\PPO} & \makecell[l]{\textbf{0.007\%}\\0.012\%}  & \makecell[l]{\textbf{0.011\%}\\0.017\%} & \makecell[l]{\textbf{0.22\%}\\0.59\%} \\
\midrule 
 \makecell[l]{$\varepsilon $-TRPO\\TRPO} & \makecell[l]{\textbf{0.014\%}\\0.015\%} & \makecell[l]{\textbf{0.67\%}\\0.69\%} & \makecell[l]{1\%\\\textbf{0.8\%}}  \\
\midrule 
 \makecell[l]{$\varepsilon $-PPOLagr\\PPOLagr} &\makecell[l]{\textbf{0.006\%}\\0.013\%} & \makecell[l]{\textbf{0\%}\\0.05\%} & \makecell[l]{\textbf{0.012\%}\\0.1\%}  \\
\midrule 
 \makecell[l]{$\varepsilon $-TRPOLagr\\TRPOLagr} & \makecell[l]{0.0004\%\\\textbf{0.00005\%}} & \makecell[l]{\textbf{0.007\%}\\0.012\%} & \makecell[l]{\textbf{0.46\%}\\0.48\%}  \\
\midrule 
\end{tabular}

%\caption{Mean \textit{violation rate} during 25 epochs of training considering TRPO, PPO, PPOLagr, TRPOLagr, and the respective \ourmethod\;version using different random seeds.}
 \label{tab:resultsFV}

